CultureMINE: Datasets and Methods for Improving the Cultural Capabilities of NLP Systems

In recent years, there has been a surge of interest in Cultural NLP, with substantial efforts to create globally inclusive NLP systems. The rapid growth of literature in this field makes it difficult to track trends in methods and data resources. To address this, we analyze over 375 papers to answer three complementary questions: (1) What Cultural Capabilities (CCs) are being targeted in NLP systems? (2) How are cultural data resources being created? and (3) What methods are being used to improve the CCs of those systems? We discuss trends observed across the three questions, and identify relevant research gaps. To facilitate further research in this field, we release our full list of analyzed papers in the form of an interactive web interface, which includes a feature to allow researchers to add their work; we hope this facilitates future research and proves to be a valuable resource for the Cultural NLP community.

==> figures/cc_table.tex <==
\begin{table*}[t]
\centering
{\small
\hyphenpenalty=10000
\exhyphenpenalty=10000
\begin{tabular}{p{0.175\linewidth} p{0.775\linewidth}}
\hline
\textbf{Cultural Capability} & \textbf{Description} \\
\hline
Cultural Translation & The capability of converting text in one language to another while preserving or accounting for cultural nuance and artifacts. \\

Survey-based Cultural Alignment & The capability of predicting the distributions of answers to value surveys conditioned on particular cultures (e.g., World Value Survey). \\

Value-driven Cultural Alignment & The capability to behave in such a way that agrees with a particular culture's values, or to switch between behaviors aligning with target cultures. \\

Cultural Knowledge & The ability to know, recall, understand, and use textual knowledge about a particular culture or cultures. \\

Multimodal Cultural Knowledge & The ability to know, recall, understand, and use visual knowledge about a particular culture or cultures. \\

Sociolinguistic Competence & The ability to understand, produce, or use language in such a way that it aligns with a particular culture or cultures' expected linguistic behavior. \\

Cultural Safety \& Harm Reduction & The ability to understand, censor, correct, or avoid text that contains harms or potential harms in accordance with a target culture or cultures. \\

Cultural Education & The capability to aid in educative processes, conditioned on a target culture or cultures. \\

Computational Cultural Representation & The capability to computationally represent, compare representations, modify representations, or edit representations of culture or features of a culture. \\
\hline
\end{tabular}
}
\caption{Descriptions of cultural capabilities in artificial intelligence.}
\label{tab:cultural_capabilities}
\end{table*}
